Location analysis of players in UEFA EURO 2020 and 2022 using generalized valuation of defense by estimating probabilities

Analyzing defenses in team sports is generally challenging because of the limited event data. Researchers have previously proposed methods to evaluate football team defense by predicting the events of ball gain and being attacked using locations of all players and the ball. However, they did not consider the importance of the events, assumed the perfect observation of all 22 players, and did not fully investigated the influence of the diversity (e.g., nationality and sex). Here, we propose a generalized valuation method of defensive teams by score-scaling the predicted probabilities of the events. Using the open-source location data of all players in broadcast video frames in football games of men's Euro 2020 and women's Euro 2022, we investigated the effect of the number of players on the prediction and validated our approach by analyzing the games. Results show that for the predictions of being attacked, scoring, and conceding, all players' information was not necessary, while that of ball gain required information on three to four offensive and defensive players. With game analyses we explained the excellence in defense of finalist teams in Euro 2020. Our approach might be applicable to location data from broadcast video frames in football games.

==> Generalized VDEP (IJPAS)/Supplementary_materials.tex <==
\newif\ifarxiv
%\arxivtrue
\arxivfalse 

\ifarxiv
\renewcommand{\thesection}{\Alph{section}}
\setcounter{section}{0}
\setcounter{figure}{0}
\setcounter{table}{0}
\else

% \documentclass[]{interact}

% \usepackage{epstopdf}% To incorporate .eps illustrations using PDFLaTeX, etc.
% \usepackage[caption=false]{subfig}% Support for small, `sub' figures and tables
%\usepackage[nolists,tablesfirst]{endfloat}% To `separate' figures and tables from text if required
%\usepackage[doublespacing]{setspace}% To produce a `double spaced' document if required
%\setlength\parindent{24pt}% To increase paragraph indentation when line spacing is doubled

% \begin{document}
\fi
\if0
\section*{}
\vspace{20mm}
\Large{\bf{Supplementary materials for: \\
\\

\noindent Location analysis of players in men’s Euro 2020 and women’s Euro 2022 using generalized valuation of defense by estimating probabilities} }

\vspace{10mm}
\ifarxiv
\noindent\large{Rikuhei Umemoto and Keisuke Fujii}
\else
\noindent\large{Anonymous}
\fi
\fi

\newpage
% \section*{Text 1. Details of ....}
% \section{Supplementary Figures}

% 下記を参考に修正する

% The number of people
% ----FIGURE START-------------------------------
\begin{figure}[h]  %b:bottom下 [t]:top上
    \begin{center}
    \vspace{30pt}
    \includegraphics[scale=0.7]{fig/histogram.png}	
    \caption{
    {\bf The number of players in broadcast videos of Euro 2020 and Euro 2022.}
    This figure shows how many players there were in broadcast videos of (a) Euro 2020 and (b) Euro 2022. 
    There were no players in some scenes. 
    In this study, to calculate the probabilities of the predictions, we removed the data (12,262 in Euro 2020 and 28,218 in Euro 2022) that did not have any player in a scene.
    } 
    \label{fig:environment}
    \end{center}
    %\vspace{-10pt}
\end{figure}
% ----FIGURE END-------------------------------

\newpage

% F1scores about euro 2022
% ----FIGURE START-------------------------------
\begin{figure}[h]  %b:bottom下 [t]:top上
    \centering
    \includegraphics[scale=0.8]{fig/f1scores_euro2022.png}
    \caption{
    {\bf F1-scores of the predictions for n\_nearest in Euro 2022.} 
    Box plots represent F1-scores of the predictions of (a) scores, (b) concedes, (c) gains and (d) attacked for n\_nearest in Euro 2022.
    As with Figure \ref{fig:f1scores_euro2020}, a green triangle means an average of F1-score at each n\_nearest and x is an outlier at a n\_nearest.
    In particular, (c), F1-scores stop to increase when n\_nearest is 3 or 4 like Euro 2020.
    }
    \label{fig:f1scores_euro2022}
\end{figure}
% ----FIGURE END-------------------------------

\newpage

% valuations about Euro 2022
% ----FIGURE START-------------------------------
\begin{figure}
    \centering
    \includegraphics[scale=0.65]{fig/valuations_2022.png}
    \caption{
    {\bf Defensive evaluations of teams in multiple games of Euro 2022.}
    Plots represent the relationship between (a) $gain\_value$ and $attacked\_value$ ($r_{14} = 0.156, p = 0.712$), (b) concedes and GVDEP values ($r_{14} = -0.557, p = 0.151$), (c) $attacked\_value$ and GVDEP values ($r_{14} = 0.999, p = 3.39\times 10^{-9}$), (d) concedes and $gain\_value$ ($r_{14} = -0.116, p = 0.784$) regarding last 8 teams of Euro 2022.
    The details about each axis were already explained in Figure \ref{fig:valuations2020}.
    As with England that was one of the finalists of Euro 2020, Germany Women's that was one of the finalists of Euro 2022 took high values for $gain\_value$ and $attacked\_value$.
    Also, similar to Italy that was another finalist of Euro 2020, another finalist of Euro 2022, England Women's, was able to keep their opponents from penetrating into the penalty area.
    These would be connected with a less number of concedes (see also Figure \ref{fig:valuations2022}b).
    }
    \label{fig:valuations2022}
\end{figure}
% ----FIGURE END-------------------------------

\newpage

% Toda's valuations about Euro 2020 & 2022
% ----FIGURE START-------------------------------
\begin{figure}[h]  %b:bottom下 [t]:top上
    \begin{center}
    \vspace{30pt}
    \includegraphics[scale=0.65]{fig/valuations_2020_toda.png}	
    \caption{
    {\bf Defensive evaluations of teams in multiple games of Euro 2020 in the definition of \cite{toda2022evaluation}.}
    Plots representing the relationship between (a) $P_{gains}$ and $P_{attacked}$ ($r_{14} = -0.135, p = 0.617$), (b) concedes and VDEP values ($r_{14} = -0.110, p = 0.686$), (c) $P_{attacked}$ and VDEP values ($r_{14} = -0.669, p = 0.00463$), (d) concedes and $P_{gains}$ ($r_{14} = 0.0333, p = 0.903$) regarding last 16 teams of Euro 2020.
    he grey lines are the averaged values of each graph's axes. 
    For $P_{gains}$, the more points plotted to the right, the more likely a team could be to gain the ball.
    Yet, for $P_{attacked}$, the more points plotted to the left or the below, the less likely an opposite team could be to attack effectively.
    Otherwise, the axes are the same meanings as Figure \ref{fig:valuations2020}.
    VDEP value that was proposed by \cite{toda2022evaluation} is calculated as follows: $P_{gains} - C \times P_{attacked}$.
    Since $C$ value is based on the number of occurrences of ball gains and being attacked,  this varies with the data ($C = 0.313$ in this study).
    } 
    \label{fig:res_testdata}
    \end{center}
    %\vspace{-10pt}
\end{figure}
% ----FIGURE END-------------------------------

% \end{document}
